Dark matter relic density from conformally or disformally coupled light scalars

Thermal freeze-out is a prominent example of dark matter (DM) production mechanism in the early Universe that can yield the correct relic density of stable weakly interacting massive particles (WIMPs). At the other end of the mass scale, many popular extensions of the Standard Model predict the existence of ultra-light scalar fields. These can be coupled to matter, preferentially in a universal and shift-symmetry-preserving way. We study the impact of such conformal and disformal couplings on the relic density of WIMPs, without introducing modifications to the thermal history of the Universe. This can either result in an additional thermal contribution to the DM relic density or suppress otherwise too large abundances compared to the observed levels. In this work, we assume that the WIMPs only interact with the standard model via the light scalar portal. We use simple models of fermionic or scalar DM, although a similar discussion holds for more sophisticated scenarios, and predict that their masses should be between $\sim 100~\textrm{GeV}$ and several $\textrm{TeV}$ to comply both with the DM abundance and current bounds on the couplings of the light scalars to matter at the LHC. Future searches will tighten these bounds.

==> header.tex <==
\RequirePackage[colorlinks=true
,urlcolor=blue
,anchorcolor=blue
,citecolor=blue
,filecolor=blue
,linkcolor=blue
,menucolor=blue
,linktocpage=true
,pdfproducer=medialab
,pdfa=true
]{hyperref}

\bibliographystyle{utphys}
%\allowdisplaybreaks

\usepackage{amsmath,amssymb,amsthm,amsfonts}
\usepackage{graphicx,tabularx}
\usepackage{color}
\usepackage{multirow}  
\usepackage{comment}
\usepackage{slashed}
\usepackage{enumitem}
\usepackage{cleveref}
\usepackage{rotating}
\usepackage[english]{babel}
\usepackage[justification=centerlast]{caption}
\usepackage{subcaption}
\usepackage{float}
%\usepackage{mathabx}
%\usepackage{pythonhighlight} 

\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{<-> mathx10}{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareMathAccent{\widebar}{0}{mathx}{"73}

\crefname{section}{Sec.}{Secs.}
\crefname{figure}{Fig.}{Figs.}
\crefname{equation}{Eq.}{Eqs.}
\crefname{appendix}{Appendix}{Appendices}
\setlist[description]{leftmargin=0.4cm}
\setlist[itemize]{leftmargin=0.4cm}

\newcommand{\be}{\begin{equation}\begin{aligned}}
\newcommand{\ee}{\end{aligned}\end{equation}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}

\newcommand{\ifb}{\text{fb}^{-1}}
\newcommand{\iab}{\text{ab}^{-1}}
\newcommand{\ev}{\text{eV}}
\newcommand{\kev}{\text{keV}}
\newcommand{\mev}{\text{MeV}}
\newcommand{\gev}{\text{GeV}}
\newcommand{\tev}{\text{TeV}}
\newcommand{\fb}{\text{fb}}
\newcommand{\pb}{\text{pb}}
\newcommand{\mb}{\text{mb}}
\newcommand{\mm}{\text{mm}}
\newcommand{\cm}{\text{cm}}
\newcommand{\m}{\text{m}}
\newcommand{\g}{\text{g}}
\newcommand{\km}{\text{km}}
\newcommand{\second}{\text{s}}
\newcommand{\mrad}{\text{mrad}}
\newcommand{\murad}{\mu\text{rad}}

\renewcommand{\eqref}[1]{Eq.~(\ref{#1})}
\newcommand{\secref}[1]{Sec.~\ref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}

\newcommand{\etal}{{\em et al.}}
\newcommand{\eg}{{\em e.g.}}
\newcommand{\ie}{{\em i.e.}}

\newcommand{\sla}[1]{\not{\! #1}}
\newcommand{\slas}[1]{\! \not{\! \! #1}}
\newcommand{\slass}[1]{\! \not{\! #1}}

\newcommand{\Seb}[1]{\textcolor{blue}{ST:#1}}
\newcommand{\Carsten}[1]{\textcolor{red}{LR:#1}}
\newcommand{\Philippe}[1]{\textcolor{green}{KJ:#1}}

\RequirePackage[normalem]{ulem}
\newcommand{\changed}[2]{{\protect\color{red}\sout{#1}}{\protect\color{blue}\uwave{#2}}}

\makeatletter
\def\l@subsubsection#1#2{}
\makeatother
